MattockFS; Page-cache and access-control concerns in asynchronous message-based forensic frameworks on the Linux platform

In this dissertation the feasibility of creating a page-cache efficient storage- and messaging solution with integrity geared access control for a scalable forensic framework is researched. The Open Computer Forensics Architecture (OCFA),a lab-side scalable computer forensics framework, introduced the concept of a message passing concurrency based forensic framework. Since then, the amount of per-investigation data to be processed in a lab environment has continued to grow significantly while available RAM and CPU processing power combined with prohibitive cost and limited capacity of SSD solutions have shifted processing from being largely CPU constrained to being much more IO constrained. OCFA suffered from several page-cache-miss related performance issues that have grown more significant as a result of this shift. In the light of anti-forensics and general issues related to process integrity, OCFA did not leverage the power of its message passing based design to address integrity concerns. The main purpose of this dissertation is to analyze and evaluate a number of page-cache friendly technologies that could contribute to the creation of a computer forensics lab-geared scalable message-passing-concurrency based forensic framework with a significantly reduced quantity of page-cache-miss induced spurious IO operations, taking into account integrity related issues. Provenance logs from historic investigations conducted using the Open Computer Forensics Architecture were thoroughly analyzed in this study, during which several bottlenecks and design flaws in OCFA were identified. A number of strategies were devised to address these bottlenecks in future computer forensic frameworks. Finally, the most prominently page-cache related strategies were consolidated with access-control measures into a user-space file-system and low-level API prototype.

==> MattockFS-mattockfs.tex <==
\chapter{MattockFS}
In this appendix we describe the functionality and design of a new user-space file-system. MattockFS is meant to be a successor to the user space file-system named CarvFS that was released by the Dutch National Police to act as an annotation based pseudo file-system aimed at facilitating zero-storage carving to the OCFA forensic framework. While CarvFS was retrofitted to work with OCFA, with MattockFS we aim to create a new user-space file-system modeled partially after CarvFS that should act as the potential foundation of new message passing oriented forensic framework. We envision that MattockFS, together with a shared key/value store,a serialization library and OCFA-Anycast like message bus technology could form the foundation for an envisioned future \emph{Mattock} forensic framework. The aim is to implement as much as is logical and sensible of the main aspects of disk-cache optimization techniques into this user space file-system. This should include facilities for querying throttling relevant information, facilities for keeping track of \emph{active} CarvPaths, facilities for marking expected read-access patterns for a given CarvPath and for marking a CarvPath as no longer needed. Also it shall include facilities for opportunistic hashing. Finally, while in OCFA, the concept of a growing archive was implemented by allowing a data-generating module access to the raw data-file underlying the file-system, in MattockFS we shall opt to implement this trough a file-system layer. This file-system should have the potential of becoming one of the foundational stones for the construction of a next generation open source message-passing concurrency based computer forensics framework. We shall refer to this envisioned framework that will need to interact closely with MattockFS as the Mattock framework or i\emph{Mattock} for short.
\section{FUSE: File-system in user-space}
In Linux, a file-system will normally reside in kernel-space. Sometimes statically as part of the main kernel, and often as a kernel loadable module. While from a performance point of view, kernel-space file-systems are preferable, writing software to run in kernel space is quite challenging and comes with many pitfalls. Most software libraries that are available in user-space are unavailable in kernel-space, and even much of the standard OS API functionality is not accessible in the same familiar and convenient access patterns. next to these concerns, there are security implications to the concept of running a large body of programming logic at the level of a trusted kernel module. As an alternative to kernel level file-systems, the Linux kernel comes with a special file-system loadable module and an accompanying user-space library that together are aptly named FUSE. FUSE is an almost-acronym that stands for Filesystem in User-space. The kernel module communicates with the library and together they allow the creation of a regular user-space process that performs the task of being a file-system. MattockFS, like CarvFS before it, aims to be such a user-space file-system. 
\section{MattockFS functionality}
MattockFS aims to become a successor to CarvFS, implementing the facilities needed for doing zero-storage (also  named "in place") file carving within the context of a computer forensic framework as CarvFS did, but also implementing a range of functionalities that aid in reducing the page-cache-miss-rate for the Mattock framework that it facilitates. Next to this, MattockFS shall implement some facilities relating to mutable data access that should contribute to the overall robustness of the framework and the integrity of the forensic process.
\subsection{The concept of concurrent pseudo-batches}
While processing of data in a forensic frameworks is something quite dynamic, when seen from MattockFS we can look at it as a large number of concurrent pseudo-batches. Each batch works on one specific piece of data as designated by one specific CarvPath. A batch consists of a set of operations on the data, each operation done by one specific framework module. A set of operations that has a beginning and an end. As such, from the point of view of the file-system, the framework and the file-system cooperate in completing pseudo-batches that are designated with the same CarvPath that also designates the data that the batch works upon. This concept of pseudo-batches is an important concept in each of the sub-responsibilities of MattockFS.
\subsection{Adding data to the archives}
In OCFA the concept of a \emph{growing archive} was introduced. The idea of a growing archive is that a large raw data file is made available through a filesystem like CarvFS of MattockFS, and that data entry processes (called kickstarts in OCFA) and data derivation processes (called dissectors in OCFA) are allowed to \emph{grow} the underlying raw data file that the file-system runs on top of. One major drawback of this approach was that the growing archive would need to be writable to each and every data producing kickstart or dissector (or as in OCFA, each and every module). Each module, or tool invoked by a module, then has the power not only to add new data to the archive, but also to potentially corrupt the existing archive. Given the reality of both anti-forensics and of software bugs in many data processing tools that might be used from within the context of a forensic framework, this approach is undesirable from a robustness and data integrity point of view. To alleviate this concern, MattockFS will implement an add-only interface for allowing Mattock modules to enter or derive data without being able to modify any of the data that was entered into the filesystem at an earlier point. Not only for data that was entered by other modules but even to the extend of not allowing mutable state to exist in any data that was fully submitted by the same module itself. MattockFS shall ensure both exclusivity of access during creation and immutability of data after it has first been fully submitted by its creator.
\subsection{Annotation based data access}
As in CarvFS, the core of the functionality of MattockFS is centered around the concept of annotation based access to data. CarvFS defined a convention for annotations named CarvPath that MattockFS will be adopting. This convention can be summarized as:
\begin{itemize}
\item CarvPath annotations can be nested like directories separated by a directory separation character as defined for the particular OS. For Linux that character is '/'. In a multi layered CarvPath, each level designates a CarvPath relative to the directory level above it. MattockFS (like CarvFS before it) will \emph{flatten} all multi-level CarvPath annotations by representing second level CarvPath entities as symbolic links to their first level \emph{flattened} representation.
\item Each CarvPath annotation comes in two forms. The \emph{directory} form that consists of just the CarvPath without a file extension, and the \emph{raw} form that is denoted using the same CarvPath, but postfixed with the \emph{.crv} file name extension.
\item A CarvPath can denote a fragmented entity within its parent. In such a case, the character '\_' is used as a separator between the fragments.
\item A \emph{normal} fragment consists of two decimal numbers separated by a \emph{'+'} sign. The first represents the offset within the parent entity. The second number denotes the size of the fragment.
\item A fragment can be defined as being \emph{sparse}. This means there is no actual data there, and if the data is read, all zeroes will be returned. A \emph{sparse} fragment is denoted as a capital \emph{'S'} followed by the size of the sparse fragment in decimal form.
\item A CarvPath may end up being longer than the OS file-system allows a directory level to be. For that reason a CarvPath annotation for a really long very fragmented CarvPath may be replaced with a digest of the CarvPath. Such a digest/CarvPath mapping will need to be stored in order to allow usage of the digest for accessing the underlying data. Note that this aspect of CarvPath annotations creates a challenge for distributed usage of CarvPath annotations. We shall discuss these concerns further down below.  
\end{itemize}
\subsection{Framework usage vs interactive usage}
The initial version of MattockFS prioritizes usage from within a framework context over interactive usage. As such performance in the interactive usage of MattockFS could be sub-optimal. It is recognized that in a real operational environment the interactive usage and framework usage will often occur simultaneous and may thus intervene with each-other. This is left as a subject for further study that falls outside of the context of this research project. We shall act as if interactive usage of MattockFS will be rare. We shall focus on MattockFS usage from within the context of pseudo-batches. Optimization of non-pseudo-batch usage is considered as an important subject, yet a subject that is not within scope for this research project.
\subsection{Page usage control, monitoring \& release}
MattockFS, when looking at it from a distance, is nothing more than a fancy wrapper for an open file handle to a huge (growing) raw archive-file. MattockFS will try to, using the \emph{fadvice} API as described in the previous appendix, in order to communicate with the kernel about keeping or no longer keeping pieces of the huge raw archive-file in the page-cache. So when should MattockFS mark a certain section of our archive to be kept or released from the page-cache? Its a quite delicate process involving reference counting, pseudo-batch marking and the opening and closing of pseudo files within the file-system. A brief outline of a simple strategy:
\begin{itemize}
\item When a batch is marked, all space indicated by the batch has a \emph{WILLNEED} reference counter incremented.
\item When a batch is unmarked, all space indicated by the batch has a \emph{WILLNEED} reference counter decremented.
\item When a pseudo file is opened, all space indicated by the pseudo file  has a \emph{NORMAL}  reference count incremented.
\item When a pseudo file is closed, all space indicated by the pseudo file has a \emph{NORMAL} reference count decremented.
\item Whenever needed, fadvice is invoked for an area resulting from reference counter values. The last \emph{advice} for any given region needs to be;
\begin{itemize}
\item \(WILLNEED == 0 ; NORMAL == 0 \Rightarrow FADV\_DONTNEED \)
\item \(WILLNEED == 0 ; NORMAL > 0 \Rightarrow FADV\_NORMAL \)
\item \(WILLNEED > 0 \Rightarrow FADV\_DONTNEED \)
\end{itemize} 
\end{itemize}
MattockFS will be keeping track of these reference counters, and as such will be able to keep track of what it has asked the kernel to keep in page cache. This information will proof useful for our throttling control later on.
\subsection{Throttling control}
While MattockFS itself does not concern itself with throttling, it is in a unique position to provide data providers within the Mattock framework with information that should proof useful then implementing effective throttling strategies. The throttling related bookkeeping in MattockFS consists of three distinct parts:
\begin{itemize}
\item The file-system provides information on the total amount of file fragment that are marked as FADV\_DONTNEED or FADV\_NORMAL.
\item As MattockFS handles read operations, and as the kernel provides the \emph{mincore} API call for checking if a page to be read resides in the page cache, MattockFS provides information as to the recent success rates with regards to page cache hits.
\item A data producing module may issue a \emph{what if} query regarding a CarvPath. This query will return the expected growth in page-cache demand resulting from consecutive marking of the CarvPath as a pseudo-batch.
\end{itemize}
The combination of these three sources of information from MattockFS should allow the modules in the framework to delay marking new pseudo-batches until old pseudo-batches have completed, possibly by throttling using the messaging subsystem.
\subsection{Opportunistic hashing}
Next to the whole \emph{fadvice} and throttling part, the concept of pseudo-batches also comes into play when implementing our opportunistic hashing. Whenever the combination of the two reference counters goes from zero to one, an opportunistic hashing context is initiated and an offset is initiated at zero. Now whenever, during the lifetime of the batch, a piece of data is read that roughly connects to the offset location, than an opportunistic hashing operation that hashes part of the data and forwards the hashing offset is attempted. If the connection isn't seamless but close, \emph{mincore} is used to check if the intermediate space happens to already be in page cache. Further, the pages directly following the requested data are also checked using the \emph{mincore} operation. Whatever chunk of in-core data can move the hashing offset forward will be used to do so.
\subsection{Distributed access concerns}
Given that MattockFS at its basis is an overlay file-system, much of the distributed access can be addressed by storing the raw archive file on an underlying file-system with distributed access. This could be something like a StorNext File System (SNFS) that allows multiple servers fiber channel access to the same data, or something like a simple NFS share. This part falls outside of the scope of concern for MattockFS.
There is however one essential distribution concern not directly related to distributed file-systems: The digest representation of long CarvPath annotations. We shall make sure that MattockFS allows for a loosely coupled link to a key/value store system that is usable in a distributed setting. A system such as \emph{Redis} would appear like a good match for such functionality. 
\section{Basic directory structure}
MattockFS uses the following base directory structure:
\begin{itemize}
\item \emph{data.crv} : A pseudo file representing the entire archive.
\item \emph{data/} : The top level for CarvPath access to the data.
\item \emph{mattockfs.info} : Empty pseudo file for file-system level interaction.
\item \emph{newdata/} : Pseudo directory for entering new data.
\end{itemize}
The data.crv file and data/ directory work in exactly the same way that CarvFS did. Nested CarvPath annotations redirect to first level flattened CarvPath annotations that are than accessible as pseudo files. What is different about the data directory is that the pseudo files inside of it allow for a close interaction of the framework using MattockFS with the throttling, page-cache management and opportunistic hashing logic inside of MattockFS and indirectly with the page-cache control functionality within the Linux Kernel. This interaction is done through the use of an extended attribute based control mechanism. Some interactions don't make sense on a per-CarvPath basis and are done against the MattockFS file-system as a whole. For that reason the pseudo file mattockfs.info acts as a front for MattockFS as a whole. This file comes with its own distinct extended attributes. Finally the directory newdata. This directory allow each distinct process accessing MattockFS to create a new pseudo file what's content is to be appended to the growing archive underlying the file-system. 
\section{CarvPath level attribute based control and info}
At the level of individual CarvPath annotations, extended attributes are to be used to interact with MattockFS. We define the following attributes:
\begin{itemize}
\item \emph{batch} : Settable boolean variable denoting if framework or script will access this CarvPath again with an other module soon. If \emph{true} MattockFS will attempt to have the kernel keep the accessed part of this CarvPath in the page-cache until set to \emph{false}. Setting \emph{batch} to \emph{true} will also initiate opportunistic hashing for the CarvPath.
\item \emph{advise}: Read only value denoting the currently set \emph{advice} value as set for the CarvPath.
\begin{itemize}
\item \emph{normal}: Set to POSIX\_FADV\_NORMAL
\item \emph{willneed}: Set to  POSIX\_FADV\_WILLNEED
\item \emph{dontneed}: Nothing set or explicitly set to POSIX\_FADV\_DONTNEED.
\item \emph{ambiguous}: Different parts of this CarvPath have a different status.
\end{itemize} 
\item \emph{incore} This attribute represents two distinct operations. When read, this variable will return a boolean indicating if the CarvPath is available in full from the page-cache. When set to \emph{true}, the CarvPath is set to POSIX\_FADV\_WILLNEED and the \emph{readahead} system API is invoked to read any uncached file data into the page-cache. This write operation will only be honored when invoked while a batch is active for this CarvPath. 
\item \emph{refcount} : This read-only attribute returns two semicolon separated integers denoting the number minimum and maximum reference count for fragments within the CarvPath indicated. If an ISO image containing a mailbox containing an individual mail is processed and all three levels are still active, requesting \emph{refcount} for the ISO image should yield \emph{1;3}, for the mailbox: {2,3} and for the individual mail \emph{3;3}. This functionality is meant for debug purposes only. 
\item \emph{throttle} : This read-only attribute returns two semicolon separated numbers indicating the price (page-cache wise) of submitting a specific CarvPath. The two numbers returned are:
\begin{itemize} 
\item The \emph{current} size of the total archive fragments for what \emph{fadvice} was invoked with a last value other than POSIX\_FADV\_DONTNEED. 
\item The total size of the additional fragments that will be marked if a batch is actively marked or the CarvPath is opened as a file. 
\end{itemize}
The result of this information is to be used for throttling purposes by the Mattock library.   
\item \emph{hash} : If fully hashed, this read-only attribute contains the 64 character hexadecimal representation of either the BLAKE2bp hash, or the SHA1 hash of the data. If both sha1 and BLAKE2 are enabled, the value here will be the BLAKE2bp hash. Until the CarvPath is fully hashed, this attribute will not be available yet.
\item \emph{sha1} :If fully hashed, this read-only attribute contains the 40 character hexadecimal representation of the 20 byte SHA-1 hash of the data. While use of SHA-1 is believed soon to become deprecated, within computer forensics systems the use of SHA-1 based, accepted and widely used data sets still depend on SHA-1. If MattockFS has SHA1 disabled than this attribute will not be available. Until the CarvPath is fully hashed, this attribute will not be available yet.
\item \emph{offset} : If not fully hashed yet, this read-only attribute contains the offset of the first byte in the file not sequentially read yet by the opportunistic hashing engine. If a hash is required from the file-system, a user can simply read the remainder of the file stating at the indicated offset. After the whole remainder of the file has been processed, the \emph{b2b} or/and \emph{sha1} attribute will be set appropriately.
\end{itemize}
\section{File-System level attribute based control}
While most interaction between MattockFS and the framework using it, will go through CarvPath annotated pseudo files, a limited set of information exists only at a file-system level. This is done using the extended attributes of the pseudo file \emph{mattockfs.info}. The following attributes are defined:
\begin{itemize}
\item \emph{size} : Read only attribute denoting the size of the \emph{fadviced} file fragments that have not \emph{yet} been set to DONTNEED.
\item \emph{normalsize} : Read only attribute denoting the size of just the \emph{fadviced} file fragments that have been explicitly marked as NORMAL. This excludes the space advised at WILLNEED level.
\item \emph{pcwillneed} : Read only attribute denoting the size of the \emph{fadviced} file fragments that have been explicitly marked as WILLNEED. This excludes the space advised at NORMAL level.
\item \emph{batchcount} : Read only attribute denoting the current number of active batch markings for CarvPath annotations.
\item \emph{filecount} : Read only attribute denoting the current number of open pseudo files for CarvPath annotations.
\item \emph{hashingcount} : Read only attribute denoting the current number of incomplete non abandoned opportunistic hashing state objects.
\item \emph{algorithms} : Read only attribute that returns the names of the hashing algorithms that have currently been configured.
\end{itemize}
\section{Creating new files}
The way to create new content in MattockFS is the creation of a specially named file in the \emph{newdata} directory. The file needs to have a CarvPath like name starting with '0+' followed by the size that needs to be allocated for this file. The file should have one of two extensions. If the file is to, once submitted, be implicitly marked as a pseudo batch, than the file extension '.bat' should be used. This should be default in-framework behavior. If however no implicit  batch context is required, than '.new' should be the file extension. A kickstart operation or derivation of data should take the following steps:
\begin{itemize}
\item Determine the size of the target file and calculate a proper file name. For example \emph{newdata/0+43246.bat} .
\item Open the file for writing.
\item Fill the non-sparse parts of the data, staying within the bounds of the claimed space.
\item Close the file.
\item After closing the file is now represented as a symbolic link. Read and dereference the symlink.
\item Delete the file.
\end{itemize} 
Note that the newdata directory is process id bound. The file is writable only to the process that created it and the symlink must be dereferenced as symlink and unlinked by that same process. While this may be inconvenient in combination with bash scripts, this setup assures the robustness of the system and immutability properties of the created data. Future versions of MattockFS may add supports for initially unknown file-size data submission. For the context of this research project however this feature falls outside of the scope.


==> ocfa-intro.tex <==
\chapter{Inter-disk-io timing in OCFA}
This appendix describes the fact-finding case-study regarding inter-job timing in the Open Computer Forensics Architecture (OCFA). While use and development of OCFA has been discontinued by the Dutch National Police, in the period from 2004 until 2012. The organization made extensive use of this asynchronous computer forensic framework. While no longer active, some old database backups were still available at the time of this study, and timing information has been extracted from these database dumps in order to study the real life disk access properties of such an asynchronous architecture. This appendix gives some background information on the OCFA messaging and routing mechanisms and on those facilities that OCFA implemented in order to prioritize processing of certain data in an attempt to optimize throughput. 
It then goes on to evaluate the timing information as extracted from the database dumps from five distinct investigations, and will try to reason about some possible explanations regarding the results of the analysis. This chapter will end with conclusions about the effectiveness of the OCFA throughput measures and areas of concern regarding disk-cache misses as far as these are relevant to the subject of this dissertation.
\section{Key points about the OCFA Architecture}
\subsection{Reasons for the asynchronous design}
In computer forensic frameworks concurrency and parallelism are important aspects. Many computer forensic tasks, such as Optical Character Recognition (OCR) of scanned documents are CPU intensive, while others like creating a full-text search-able index are IO-intensive and some like the calculation of hashes of data are both. There is a tension between optimizing a forensic framework for IO efficiency and optimizing it for the effective use of available CPU power. There is also a tension between optimizing a forensic framework for single-node performance and making the framework scale to make use of a cluster of workers for CPU intensive tasks. When we look at the base idea of concurrency, there are two models by which a concurrent system can operate: 
\begin{itemize}
\item Shared state concurrency.
\item Message passing concurrency.
\end{itemize}
Shared state concurrency comes with many advantages in the light of the tension between IO efficiency issues, yet message passing concurrency is fundamental better suited for the multi-server high-CPU module scenario. For OCFA it was a different non-functional requirement that tipped the scale towards the use of message passing security: \emph{robustness in the event of local failure}. OCFA was meant to be used in
a highly dynamic and reactive environment where investigations could not wait for a development team to create a robust well tested module at the moment the need arose. No, in OCFA, the use of highly targeted \emph{quick and dirty} module development was an essential feature. A feature however that meant that a module could and would occasionally just crash. Both locality of failure and crash recovery ended up being primary specifications for the OCFA architecture and the choice for message passing concurrency flowed naturally from that. A choice that as this appendix will show comes at a price.
\subsection{High-level routing of jobs}
Messaging in the OCFA framework took place at two distinct levels of abstraction. At the highest level of abstraction, meta-data was passed between module \emph{functionalities} by a process (or set of processes) called the XML-Router. This router would evaluate the meta-data generated by previous modules and would, based on that meta-data, determine what module should come next. We shall see in our results and evaluation below that some aspects of the XML-router implementation possibly ended up hindering primary performance in an important way.
\subsection{Low-level relaying of jobs}
While the high-level XML-routing was essential to the OCFA framework as messaging mechanism, and while the routing system as we shall show later on did have an impact on performance, the main message-passing concurrency system for OCFA was constituted by the low level relaying system. This system consisted of two main components:
\begin{itemize}
\item The Persistent Priority Queue library.
\item The Anycast Relay
\end{itemize}
The Anycast relay was a single process implementation of what today would be called a message bus. It shared many characteristics with modern message bus systems like RabbitMQ, yet specifically tailored for the OCFA systems robustness and crash-recovery needs. A full description of the crash-recovery features of the Anycast relay falls outside of the scope of this paper, but it is sufficient to state that the Anycast relay would set-aside unprocessed and partially processed messages from crashed module instances to both allow for localization of failure and for solid crash recovery. The Anycast relay was a simple messaging server with a persistent per module-type message-queue. Within the 
Anycast relay messaging system each module would both be consumer (based on its module functionality) and producer in a multi-producer multi-consumer set-up. 
For the purpose of this document, the Anycast Relay should be seen as a set of channels between producers and consumers or consumer pools. As is a well known problem with buffer constrained systems, asynchronous message passing systems like OCFA can suffer from situations that truly stretch the capacity needs for message buffers. The Persistent Priority Queue library solves these issues for OCFA in a way that prioritizes robustness and delivery guarantees over performance concerns. We shall later evaluate the choices made for OCFA and how changes in these choices could potentially improve the way a computer forensic framework could attenuate the buffering issue that seems to be inherent to the choice for message passing concurrency. 
\subsection{Job priorities and queuing}
The main strategy applied by OCFA in order to improve the throughput of the overall architecture is the use of priorities. We shall later see that while according to some measurements that focus on the per-event timing, these measures would seem effective, yet when focussing on other measurements, namely those for per volume timing, these measures turn out to be highly inadequate. The basic idea of the job priorities for OCFA was that each non-router module would increment the priority of the processed data. While this concept worked on a link by link basis, it did help to allow individual modules (including the router) to prioritize the oldest data, thus allowing the framework to reduce the amount of cumulative active data in the system. 
\subsection{Timestamps in the OCFA databases}
The XML Blobs created and extended by the OCFA modules don't contain just per-job meta-data. They are also used to store profiling information listing the start time and stop time of every module with a one second granularity.  These XML blobs are all stored in the Postgress database that is used as central component in the OCFA infrastructure. From this profiling information it should be possible to extract some basic statistics that should prove useful in analyzing and evaluating the disk-cache-miss likelihood and possibly come up with the most suitable remedies for improving upon these.
\section{Analysis of the OCFA timing information}
\subsection{Extracting the timing information}
The Dutch National Police made a set of database dumps from old OCFA runs available for use in this study. One important prerequisite however was that the sensitive investigative data would under no circumstances become part of the scientific research. In order to adhere to these preconditions, a Python script was created to parse the database dumps and to extract only those parts of the data that were essential for \emph{technical} evaluation related to timing. In theory this information should be sufficient to base our research and evaluations on, yet it is possible that a better foundation of our findings would be possible when including non-directly timing related information. The python script as referenced in a following appendix did the following:
\begin{itemize}
\item Extract the evidence XML blobs from the SQL dump.
\item Extract the oldest timestamp from the XML blobs and use that time as offset for the successive steps.
\item Process each individual XML blob and extract only the relative start and stop times and module types for each job.
\item Write the extracted information to a JSON based log file.
\end{itemize}
The true analysis of the OCFA timing information took place on the resulting JSON based log files. It is important to note that due to a bug in the OCFA Java library at the time these investigations were active, there are were some (detectable/reversible) offset bugs in the results. These needed to be corrected during the actual analysis.





